An Introduction to the Deviatoric Tensor Decomposition in Three Dimensions and its Multipole Representation

The analysis and visualization of tensor fields is a very challenging task. Besides the cases of zeroth- and first-order tensors, most techniques focus on symmetric second-order tensors. Only a few works concern totally symmetric tensors of higher-order. Work on other tensors of higher-order than two is exceptionally rare. We believe that one major reason for this gap is the lack of knowledge about suitable tensor decompositions for the general higher-order tensors. We focus here on three dimensions as most applications are concerned with three-dimensional space. A lot of work on symmetric second-order tensors uses the spectral decomposition. The work on totally symmetric higher-order tensors deals frequently with a decomposition based on spherical harmonics. These decompositions do not directly apply to general tensors of higher-order in three dimensions. However, another option available is the deviatoric decomposition for such tensors, splitting them into deviators. Together with the multipole representation of deviators, it allows to describe any tensor in three dimensions uniquely by a set of directions and non-negative scalars. The specific appeal of this methodology is its general applicability, opening up a potentially general route to tensor interpretation. The underlying concepts, however, are not broadly understood in the engineering community. In this article, we therefore gather information about this decomposition from a range of literature sources. The goal is to collect and prepare the material for further analysis and give other researchers the chance to work in this direction. This article wants to stimulate the use of this decomposition and the search for interpretation of this unique algebraic property. A first step in this direction is given by a detailed analysis of the multipole representation of symmetric second-order three-dimensional tensors.

==> rest.tex <==
\subsection{Mechanische Grundlagen}
 A three-dimensional fourth-order tensor $\mathbfcal{C}$ can be written as
\begin{equation}
(\mathbf{e}_i \otimes \mathbf{e}_j) : \mathbfcal{C} : (\mathbf{e}_k \otimes \mathbf{e}_l) = C_{ijkl}, \qquad i,j,k,l \in \{ 1,2,3 \}
\end{equation}
where 


A deviator is defined as a traceless tensor. Therefore the deviatoric part of a three-dimensional second-order tensor $\textbf{T}$ is given by 
\begin{equation}
\mathrm{dev}(\textbf{T}) = \textbf{T} - {{1}\over{3}}\mathrm{tr}(\textbf{T}) \textbf{I}
\end{equation}
where $\textbf{I}$ is the unit tensor. 





\subsubsection{Fourth-order tensor}
The eigenvalues of the stiffness tensor are called eigenstiffnesses.\\
\begin{itemize}
\item Spektralzerlegung
\begin{itemize}

\item Eigensteifigkeiten, Eigenspannungen, Eigenverzerrung (was ist das? Zerlegung der einzelnen Verzerrungen, addieren aller Einzelverzerrungen = Gesamtverzerrung (Helbig/Kelvin))
\end{itemize}
......................\\
\end{itemize}



\begin{comment}
\begin{itemize}
\item Generelle Darstellung
\item Stiffness-Tensor: Symmetrie durch Hook
\item Dadurch, dass $\bm{\sigma}$ und $\bm{\varepsilon}$ symmetrisch sind und aus dem Hookschen Gesetz folgt:
\item Somit nicht 81 Komponenten, sondern nur 21. 4.Ordnung Tensor mit 3 Dimensionen kann als 6dim Tensor 2. Ordnung dargestellt werden:
\item Voigt
\item Voigt Mapping erhaelt die Tensor-Norm nicht, somit ist Resultat kein Tensor mehr. 
\item Kelvin
\begin{itemize}
\item 
\begin{align}
&\bm{\sigma} = \begin{pmatrix}
\sigma_{11} & \sigma_{22} & \sigma_{33} & \sqrt{2}\sigma_{23} & \sqrt{2}\sigma_{13} & \sqrt{2}\sigma_{12}
\end{pmatrix}^T\\
&\bm{\varepsilon} = \begin{pmatrix}
\varepsilon_{11} & \varepsilon_{22} & \varepsilon_{33} & \sqrt{2}\varepsilon_{23} & \sqrt{2}\varepsilon_{13} & \sqrt{2}\varepsilon_{12}
\end{pmatrix}^T
\end{align}
\item Kelvin Mapping erhaelt die Tensornorm.
\end{itemize}
\end{comment}


\begin{itemize}
\item Symmetrieebene/Multipole
\end{itemize}
